Unsupervised Pre-Training for Vietnamese Automatic Speech Recognition in the HYKIST Project

In today's interconnected globe, moving abroad is more and more prevalent, whether it's for employment, refugee resettlement, or other causes. Language difficulties between natives and immigrants present a common issue on a daily basis, especially in medical domain. This can make it difficult for patients and doctors to communicate during anamnesis or in the emergency room, which compromises patient care. The goal of the HYKIST Project is to develop a speech translation system to support patient-doctor communication with ASR and MT. ASR systems have recently displayed astounding performance on particular tasks for which enough quantities of training data are available, such as LibriSpeech. Building a good model is still difficult due to a variety of speaking styles, acoustic and recording settings, and a lack of in-domain training data. In this thesis, we describe our efforts to construct ASR systems for a conversational telephone speech recognition task in the medical domain for Vietnamese language to assist emergency room contact between doctors and patients across linguistic barriers. In order to enhance the system's performance, we investigate various training schedules and data combining strategies. We also examine how best to make use of the little data that is available. The use of publicly accessible models like XLSR-53 is compared to the use of customized pre-trained models, and both supervised and unsupervised approaches are utilized using wav2vec 2.0 as architecture.

==> chapter/Experimental_results_03.tex <==
\section{Training time trade-offs in rapid development}

\begin{figure}[hbtp]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/pretrain_comparison.pdf}
	\caption{
	    \glsxtrshort{WER} comparison using several pre-training checkpoints fine-tuned on the same schedule. 
	    The quantity of pre-training epochs is represented on the horizontal axis. 
	    The vertical axis displays the \glsxtrshort{WER} obtained after optimizing the Vietnamese in-house system on HYKIST dev data till convergence and evaluated on the initialization checkpoint that corresponds to it. 
	    All the pre-trainings in Vietnamese have been done using in-house data, not \glsxtrshort{YT} data. 
	    Keep in mind that if utilizing as an initialization, the training epochs for that model are not taken into consideration.
	    }
	\label{fig:fine_tune_comp_joint}
\end{figure}

It is vital to identify a trade-off between training time allowed and potential system performance while constructing \glsxtrshort{ASR} systems quickly. 
In this section, we examine the models that are most useful for this purpose. 
One epoch of pre-training on our internal Vietnamese data may be assumed to take around an hour on an NVIDIA 2080 GPU, but one epoch of fine-tuning can be estimated to take about three hours on the same setup. 
In our trials, the needed pre-training time scaled linearly with the amount of data.

Figure \ref{fig:fine_tune_comp_joint} compares various training methods using a hold-out dev dataset.
Yellow represents the baseline when fine-tuning from scratch.
Although pre-training using the in-house Vietnamese data (blue) results in a tiny improvement, it converges and stops improving after 100 iterations.
This is true even when the unsupervised loss is still improving.
Contrarily, the multilingual pre-training (orange) performs much better than the monolingual pre-training and enhances downstream \glsxtrshort{WER} even over prolonged training time.

Vietnamese \textit{XLSR-53}\textsubscript{1-8} (grey) fine-tuning is a very cost-effective training method that outperforms starting from scratch or pre-training on monolingual in-house data while utilizing only 26 training epochs in total.
Please take note that since the original \glsxtrshort{XLSR-53} model is available to the public, we do not count training epochs.
Although it requires more training time, using \glsxtrshort{XLSR-53} as an initialization for additional custom pre-training results in considerable \glsxtrshort{WERR} (green, red, purple).
It is evident from Figure \ref{fig:fine_tune_comp_joint} that even a brief pre-training with a few epochs produces significant benefits.
Consequently, this can be viewed as a quick and affordable solution to improve the performance of the model.
When employing data that is multilingual, the \glsxtrshort{WERR} is very potent.
Despite the fact that we have more data in this instance and a lengthier pre-training as a result, we only need to conduct this procedure once for all languages, making the situation essentially a zero-sum game.

In conclusion, it is clear that using the \glsxtrshort{XLSR-53} model to construct high-performing \glsxtrshort{ASR} models is very cost-effective. 
A quick multilingual pre-training that is helpful for downstream fine-tuning in all languages can further enhance performance.

==> chapter/introduction.tex <==
\chapter{Introduction}
\label{ch: Introduction}

\begin{quotation}
    Please add your introductory text here.
\end{quotation}


==> header/bib_config.tex <==
\usepackage[
    backend=biber,
    citestyle=authortitle,
    bibstyle=authortitle,
    isbn=false,
    doi=false,
    url=false,
    block=space,
    maxcitenames=2,
    maxbibnames=99,
    backref=false,
    giveninits=true,
    dashed=false]{biblatex}
\setlength{\bibitemsep}{1em}
\setlength{\bibhang}{2em}

\DeclareFieldFormat[
    book,
    article,
    inbook,
    incollection,
    inproceedings,
    patent,
    thesis,
    unpublished,
    misc,
    manual]
{citetitle}{\mkbibparens{#1\isdot}}


% \usepackage[backend=biber,
%     bibencoding=utf8,
%     %citestyle=alphabetic,
%     citestyle=verbose-note,
%     bibstyle=verbose,
%     %style=verbose,
%     url=true,
%     autocite=footnote,
%     sorting=nyt, %Sortierung nach Name, Jahr, Titel
%     defernumbers=true,
%     maxbibnames=99
% ]{biblatex}


% % See https://ctan.space-pro.be/tex-archive/macros/latex/contrib/xurl/doc/xurl.pdf
% \setcounter{biburllcpenalty}{100}
% \setcounter{biburlucpenalty}{200}
% \setcounter{biburlnumpenalty}{100}

% \DeclareFieldFormat{file}{Datei: {\sloppy\url{#1}}}
% \renewbibmacro{finentry}{\printfield{file}\finentry}

% % TODO: check https://tex.stackexchange.com/a/582029/144487 for whether it is a better solution
% % Stolen from https://tex.stackexchange.com/questions/200286/biblatex-repeated-citations-in-footnotes-that-point-back-to-earlier-footnotes  
% \makeatletter
% \DeclareCiteCommand{\superfootcite}
% {}
% {\usebibmacro{citeindex}%
%     \usebibmacro{superfootcite}}
% {}
% {}

% \newbibmacro*{superfootcite}{%
%     \ifciteseen
%     {\usebibmacro{superfootcite:note}}
%     {\mkbibfootnote{\usebibmacro{footcite:full}%
%             \usebibmacro{footcite:save}}}}

% \newbibmacro*{superfootcite:note}{\footref{cbx@\csuse{cbx@f@\thefield{entrykey}}}}
% \makeatother

% % TODO: dive deeper starting here
% % https://tex.stackexchange.com/questions/319084/defbibenvironment-letters-instead-of-numbers
% \defbibenvironment{bibliography}
% {\trivlist}
% {\endtrivlist}
% {\item
%     % \printtext[labelnumberwidth]{%
%     %     \printfield{labelprefix}%
%     %     \printfield{labelnumber}%
%     % }%
%     \addspace}

% % https://tex.stackexchange.com/a/1690/144487
% \DeclareCiteCommand{\parencite}[\mkbibparens]
% {\usebibmacro{prenote}}
% {\usebibmacro{citeindex}%
%     \printtext[bibhyperref]{\usebibmacro{cite}}
% }
% {\multicitedelim}
% {\usebibmacro{postnote}}


==> misc/glossary.tex <==
\newglossaryentry{sg}
{
    name={safety goal},
    description={is a high-level safety requirement as a result of the hazard analysis and risk assessment at the vehicle level and is formulated for each hazardous event},
    type=glossaryx
}

==> misc/symbols.tex <==
\newglossaryentry{w}{name=\ensuremath{P},
    description={power},
    unit={\ensuremath{W}},
    type=symbolslist}

\newglossaryentry{mps}{name=\ensuremath{V},
    description={speed},
    unit={\ensuremath{m/s}},
    type=symbolslist}

\newglossaryentry{kmh}{name=\ensuremath{V},
    description={speed},
    unit={\ensuremath{km/h}},
    type=symbolslist}


==> tables/Lr_reset_int_loss.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}


\begin{table}[!ht]
\centering
\begin{adjustbox}{width=0.5\columnwidth,center}
\begin{tabular}{|c|c|c|cc|} 
\hline
\#Ft-Epoch          & \multicolumn{2}{c|}{Data}      & Baseline      & +IF                \\ 
\hline
\multirow{5}{*}{13} & \multirow{2}{*}{hykist} & dev  & 32.8          & \textbf{32.1}           \\ 
\cline{3-5}
                    &                         & test & 37.6          & \textbf{37.2}           \\ 
\cline{2-5}
                    & \multirow{2}{*}{cv}     & dev  & \textbf{17.0} & 17.5                    \\ 
\cline{3-5}
                    &                         & test & \textbf{39.5} & \textbf{39.5}           \\ 
\cline{2-5}
                    & \multicolumn{2}{c|}{vivos}     & 34.0          & \textbf{33.7}           \\ 
\hline
\multirow{5}{*}{33} & \multirow{2}{*}{hykist} & dev  & 32.8          & \textbf{\textbf{31.9}}  \\ 
\cline{3-5}
                    &                         & test & 37.6          & \textbf{\textbf{36.9}}  \\ 
\cline{2-5}
                    & \multirow{2}{*}{cv}     & dev  & \textbf{17.0} & 18.3                    \\ 
\cline{3-5}
                    &                         & test & \textbf{39.5} & 40.0                    \\ 
\cline{2-5}
                    & \multicolumn{2}{c|}{vivos}     & 34.0          & \textbf{33.9}           \\
\hline
\end{tabular}
\end{adjustbox}
\caption{\glspl{WER} comparison of \glsxtrshort{IF Loss} over epochs of learning rate reset training. The recognition was done on HYKIST, CommonVoice and VIVOS dataset.}
\label{Lr_reset_int_loss}
\end{table}

==> tables/encoder_compare_RawWF.tex <==
\begin{table}[!h]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Architecture} & \multirow{2}{*}{Features} & \multicolumn{2}{c|}{Pretraining}              & Fine-tuning         & \multicolumn{2}{c|}{WER [\%]}  \\ 
\cline{3-7}
                              &                           & Data (hours)          & Epochs                & Epochs              & dev  & test                    \\ 
\hline
\textit{Base}                 & \multirow{2}{*}{Raw WF}   & \multirow{2}{*}{None} & \multirow{2}{*}{None} & \multirow{2}{*}{33} & 35.8 & 39.9                    \\ 
\cline{1-1}\cline{6-7}
\textit{Large}\textsubscript{1-8}             &                           &                       &                       &                     & 35.0 & 40.7                    \\
\hline
\end{tabular}
\end{adjustbox}
\caption{\glspl{WER} {[}\%{]} for models fine-tuning from scratch. All fine-tunings use the \textit{Large}\textsubscript{1-8} or \textit{Base} architecture and are trained until full convergence on the Vietnamese in-house data. Pre-training "None" means fine-tuning from scratch. Features used are Raw Waveform (Raw WF).}
\label{table:encoder_compare_RawWF}
\end{table}

==> tables/encoder_compare_augment.tex <==
\begin{table}[!h]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Architecture} & \multirow{2}{*}{Features} & \multicolumn{2}{c|}{Pretraining}                                                                                        & Fine-tuning         & \multicolumn{2}{c|}{WER [\%]}  \\ 
\cline{3-7}
                              &                           & Data (hours)                                                                                     & Epochs               & Epochs              & dev  & test                    \\ 
\hline
\textit{Base}                 & \multirow{2}{*}{Raw WF}   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Augmented~ in-house \\dataViet. (1168h)\end{tabular}} & \multirow{2}{*}{300} & \multirow{2}{*}{26} & 31.6 & 32.2                    \\ 
\cline{1-1}\cline{6-7}
\textit{Large}\textsubscript{1-8}             &                           &                                                                                                  &                      &                     & 31.0 & 32.3                    \\
\hline
\end{tabular}
\end{adjustbox}
\caption{\glspl{WER} {[}\%{]} for models fine-tuning using augmented data for pre-training.}
\label{table:encoder_compare_augment}
\end{table}

==> tables/encoder_feature_compare.tex <==
\begin{table}[!h]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multirow{3}{*}{Architecture} & \multirow{3}{*}{Features} & \multicolumn{2}{c|}{Pretraining}                                                                                               & Fine-tuning             & \multicolumn{2}{c|}{WER [\%]}  \\ 
\cline{3-7}
                              &                           & \multirow{2}{*}{Data (hours)}                                                                        & \multirow{2}{*}{Epochs} & \multirow{2}{*}{Epochs} & \multicolumn{2}{c|}{Viet.}     \\ 
\cline{6-7}
                              &                           &                                                                                                      &                         &                         & dev  & test                    \\ 
\hline
\textit{Base}                         & \multirow{2}{*}{Raw WF}   & \multirow{3}{*}{None}                                                                                & \multirow{3}{*}{None}   & \multirow{7}{*}{33}     & 35.8 & 39.9                    \\ 
\cline{1-1}\cline{6-7}
\textit{Large}\textsubscript{1-8}                        &                           &                                                                                                      &                         &                         & 35.0 & 40.7                    \\ 
\cline{1-2}\cline{6-7}
\textit{Large}\textsubscript{1-8}                        & GT                        &                                                                                                      &                         &                         & 36.8 & 38.4                    \\ 
\cline{1-4}\cline{6-7}
\textit{Base}                         & \multirow{16}{*}{Raw WF}  & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Respective~\\in-house \\dataViet. \\(0.01h)\end{tabular}} & \multirow{4}{*}{1}      &                         & 30.6 & 35.2                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\ 
\cline{1-1}\cline{6-7}
\textit{Large}\textsubscript{1-8}                        &                           &                                                                                                      &                         &                         & 31.8 & 35.7                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\ 
\cline{1-1}\cline{3-7}
\textit{Base}                         &                           & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Respective~\\in-house \\dataViet. \\(219h)\end{tabular}}  & \multirow{12}{*}{300}   & \multirow{12}{*}{26}    & 30.2 & 33.3                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\ 
\cline{1-1}\cline{6-7}
\textit{Large}\textsubscript{1-8}                        &                           &                                                                                                      &                         &                         & 31.5 & 33.4                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\ 
\cline{1-1}\cline{3-3}\cline{6-7}
\textit{Base}                         &                           & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Multilingual \\in-house~\\(1168h)\end{tabular}}           &                         &                         & 26.2 & 28.8                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\ 
\cline{1-1}\cline{6-7}
\textit{Large}\textsubscript{1-8}                        &                           &                                                                                                      &                         &                         & 26.8 & 28.7                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\ 
\cline{1-1}\cline{3-3}\cline{6-7}
\textit{Base}                         &                           & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Augmented~\\in-house \\dataViet. \\(1168h)\end{tabular}}  &                         &                         & 31.6 & 32.2                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\ 
\cline{1-1}\cline{6-7}
\textit{Large}\textsubscript{1-8}                        &                           &                                                                                                      &                         &                         & 31.0 & 32.3                    \\
                              &                           &                                                                                                      &                         &                         &      &                         \\
\hline
\end{tabular}
\end{adjustbox}
\caption{\glspl{WER} {[}\%{]} for models using unsupervised pre-training and fine-tuning from scratch. All fine-tunings use the \textit{Large}\textsubscript{1-8} or \textit{Base} architecture and are trained until full convergence on the in-house data of the respective language. Pre-trainings have been done with random initialization. Pre-training "None" means fine-tuning from scratch. Features used are Raw Waveform (Raw WF) or Gammatone (GT) \cite{schlueter:icassp07}.}
\label{table:encoder_feature_compare}
\end{table}

==> tables/feature_compare.tex <==
\begin{table}[!h]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Architecture} & \multirow{2}{*}{Features} & \multicolumn{2}{c|}{Pretraining} & Fine-tuning & \multicolumn{2}{c|}{WER [\%]}  \\ 
\cline{3-7}
                              &                           & Data (hours) & Epochs            & Epochs      & dev  & test                    \\ 
\hline
\textit{Large}\textsubscript{1-8}             & GT                        & None         & None              & 33          & 36.8 & 38.4                    \\
\hline
\end{tabular}
\end{adjustbox}
\caption{\glspl{WER} {[}\%{]} for models fine-tuning using \glsxtrfull{GT} feature. The setup is built the same to \glsxtrshort{CNN} feature.}
\label{table:feature_compare}
\end{table}

==> tables/int_and_focal_WERs.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}


\begin{table}[!ht]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|c|} 
\hline
Arch.                              & Init                              & Pre-training data                                                                    & Recog. & Baseline      & +ICE          & +IF           & +L2           \\ 
\hline
\multirow{8}{*}{\textit{Large}\textsubscript{1-8}} & \multirow{2}{*}{\textit{XLSR-53}}          & \multirow{2}{*}{None}                                                                & dev    & \textbf{27.9} & 28.4          & 28.0          & -             \\ 
\cline{4-8}
                                   &                                   &                                                                                      & test   & \textbf{32.3} & 33.3          & 32.8          & -             \\ 
\cline{2-8}
                                   & \multirow{4}{*}{None}             & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}In-house data Viet.\\(219h)\end{tabular}} & dev    & 30.4          & 29.1          & \textbf{28.6} & 28.8          \\ 
\cline{4-8}
                                   &                                   &                                                                                      & test   & 33.4          & 33.7          & \textbf{33.0} & \uline{32.9}  \\ 
\cline{3-8}
                                   &                                   & \multirow{2}{*}{None}                                                                & dev    & 35.6          & 33.8          & \textbf{33.0} & \uline{31.4}  \\ 
\cline{4-8}
                                   &                                   &                                                                                      & test   & 40.7          & \textbf{38.1} & 38.8          & \uline{36.4}  \\ 
\cline{2-8}
                                   & \multirow{2}{*}{\textit{XLSR-53}} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}In-house data Viet.\\(219h)\end{tabular}} & dev    & 25.5          & 25.2          & \textbf{24.7} & \uline{24.3}  \\ 
\cline{4-8}
                                   &                                   &                                                                                      & test   & \textbf{29.1} & 29.2          & \textbf{29.1} & 29.3          \\ 
\cline{1-2}\cline{4-8}
\multirow{2}{*}{\textit{Base}}     & \multirow{4}{*}{None}             &                                                                                      & dev    & 30.2          & 29.7          & \textbf{29.0} & \uline{28.8}  \\ 
\cline{4-8}
                                   &                                   &                                                                                      & test   & 33.3          & 33.4          & \textbf{33.0} & \uline{32.3}  \\ 
\cline{1-1}\cline{3-8}
\multirow{2}{*}{\textit{Large}\textsubscript{1-8}} &                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Viet. YT\\(1168h)\end{tabular}}           & dev    & 29.8          & 27.3          & \textbf{26.1} & -             \\ 
\cline{4-8}
                                   &                                   &                                                                                      & test   & 35.2          & 31.5          & \textbf{30.8} & -             \\
\hline
\end{tabular}
\end{adjustbox}
\caption{
    Comparison of \glspl{WER} between architecture sizes, pretrained datasets and pretrained models, all are finetuned on our in-house spontaneous telephone speech dataset and recognized at epoch 33 on dev and test telephone HYKIST data. 
    In this table, only 1 intermediate layer is applied in the middle \glsxtrshort{Transformer} block, e.g. position 4 for \textit{Large}\textsubscript{1-8} and 6 for \textit{Base} architecture. 
    \textbf{Bold} numbers are used to compare between the baseline and 2 types of intermediate loss, while \underline{underline} numbers denote extra improvement of L2 regularization compared to \glsxtrshort{IF Loss}}
\label{int_and_focal_WERs}
\end{table}

==> tables/int_and_focal_WERs_CV_Vivos.tex <==
\begin{table}[!ht]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
Arch.                                                                      & Init                              & Pre-training data                                                                    & Recog. & Baseline      & +ICE           & +IF            \\ 
\hline
\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}\\\textit{Large}\textsubscript{1-8}\end{tabular}} & \multirow{3}{*}{\textit{XLSR-53}} & \multirow{3}{*}{None}                                                                & dev    & \textbf{14.8} & 15.8           & 15.4           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & test   & \textbf{32.5} & 33.9           & 33.6           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & vivos  & 30.3          & \textbf{30.0}  & \textbf{30.0}  \\ 
\cline{2-7}
                                                                           & \multirow{6}{*}{None}             & \multirow{3}{*}{In-house data Viet.(219h)}                                           & dev    & 16.4          & 16.1           & \textbf{15.8}  \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & test   & 35.6          & 34.8           & \textbf{34.5}  \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & vivos  & 31.3          & 30.4           & \textbf{29.6}  \\ 
\cline{3-7}
                                                                           &                                   & \multirow{3}{*}{None}                                                                & dev    & 20.8          & \textbf{18.6}  & 19.7           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & test   & 44.7          & \textbf{42.1}  & 43.1           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & vivos  & 34.9          & \textbf{33.1}  & 33.9           \\ 
\cline{2-7}
                                                                           & \multirow{3}{*}{\textit{XLSR-53}} & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}In-house data Viet.\\(219h)\end{tabular}} & dev    & \textbf{11.5} & 12.3           & 13.0           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & test   & \textbf{29.4} & 29.8           & 29.8           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & vivos  & \textbf{27.2} & 27.7           & 27.6           \\ 
\cline{1-2}\cline{4-7}
\multirow{3}{*}{\textit{Base}}                                             & \multirow{6}{*}{None}             &                                                                                      & dev    & 16.6          & \textbf{15.4}~ & 15.9           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & test   & 35.4          & \textbf{34.2}  & 34.4           \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & vivos  & 30.9          & 31.3           & \textbf{30.5}  \\ 
\cline{1-1}\cline{3-7}
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\\\textit{Large}\textsubscript{1-8}\end{tabular}}  &                                   & \multirow{3}{*}{Viet. YT(1168h)}                                                     & dev    & 16.4          & 15.6           & \textbf{14.5}  \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & test   & 34.4          & 32.2           & \textbf{30.9}  \\ 
\cline{4-7}
                                                                           &                                   &                                                                                      & vivos  & 28.7          & 27.6           & \textbf{26.9}  \\
\hline
\end{tabular}
\end{adjustbox}
\caption{
    Recognition \glspl{WER} at epoch 33 on read speech datasets. 
    Experiment setups are the same to Table \ref{int_and_focal_WERs}. 
    The recognition is done on CommonVoice dev/test sets and VIVOS test set.}
\label{int_and_focal_WERs_CV_Vivos}
\end{table}

==> tables/literature_compare.tex <==
\begin{table}[!ht]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|} 
\hline
Work              & \multicolumn{2}{c|}{\cite{Duy_Khanh_Finetune_Wav2vec_2_0_2022}}                                                                         & Our best Monoling.                                                   & Our best Multiling.                                                     \\ 
\hline
Approach          & \multicolumn{2}{c|}{End-to-end}                                                                          & \multicolumn{2}{c|}{Hybrid}                                                                                                                    \\ 
\hline
Init. model       & \multicolumn{3}{c|}{None}                                                                                                                                                       & \textit{XLSR-53}                                                        \\ 
\hline
Pretrain data [h] & \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}VLSP + CV + VIVOS \\(160h)\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}Viet. in-house + YT\\(1168h)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Multilingual in-house\\(1168h)\end{tabular}  \\ 
\cline{1-1}\cline{4-5}
Finetune data [h] & \multicolumn{2}{c|}{}                                                                                    & \multicolumn{2}{c|}{In-house dataViet. (219h)}                                                                                                 \\ 
\hline
Text data         & no                                      & 2GB                                                            & \multicolumn{2}{c|}{500M words}                                                                                                                \\ 
\hline
WER dev           & \textcolor[rgb]{0.114,0.11,0.114}{38.5} & \textcolor[rgb]{0.114,0.11,0.114}{27.4}                        & 25.3                                                                 & 23.9                                                                    \\ 
\hline
WER test          & \textcolor[rgb]{0.114,0.11,0.114}{43.1} & \textcolor[rgb]{0.114,0.11,0.114}{31.6}                        & 27.2                                                                 & 27.4                                                                    \\
\hline
\end{tabular}
\end{adjustbox}
\caption{\glspl{WER} comparison between our best monolingual/multilingual models and other wav2vec 2.0 model. \glsxtrshort{LM} of \cite{Duy_Khanh_Finetune_Wav2vec_2_0_2022} is generated by \cite{vietai_wav2vec2_vi_2021}'s model.}
\label{literature_compare}
\end{table}

==> tables/transfer_learning_strategy.tex <==
\begin{table}[!ht]
\centering
\begin{adjustbox}{width=0.9\columnwidth,center}
\begin{tabular}{|c|c|l|} 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{\textbf{Training }}\\\textbf{\textbf{size}}\end{tabular} & \textbf{\textbf{Illustration}} & \multicolumn{1}{c|}{\textbf{\textbf{Explanation}}}                                                                                                                                                                                                                                                               \\ 
\hline
\textcolor[rgb]{0.141,0.161,0.18}{Small}                                                    & \raisebox{-\totalheight}{\includegraphics[width=0.7\textwidth, height=60mm]{figures/transfer-learning-small-ltr.png}}                       & \begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.141,0.161,0.18}{Freezes all layers, }\\\textcolor[rgb]{0.141,0.161,0.18}{trains weights }\\\textcolor[rgb]{0.141,0.161,0.18}{on softmax}\end{tabular}                                                                                                               \\ 
\hline
\textcolor[rgb]{0.141,0.161,0.18}{Medium}                                                   & \raisebox{-\totalheight}{\includegraphics[width=0.7\textwidth, height=60mm]{figures/transfer-learning-medium-ltr.png}}                       & \begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.141,0.161,0.18}{Freezes most }\\\textcolor[rgb]{0.141,0.161,0.18}{layers, trains weights }\\\textcolor[rgb]{0.141,0.161,0.18}{on last layers and }\\\textcolor[rgb]{0.141,0.161,0.18}{softmax}\end{tabular}                                                         \\ 
\hline
\textcolor[rgb]{0.141,0.161,0.18}{Large}                                                    & \raisebox{-\totalheight}{\includegraphics[width=0.7\textwidth, height=60mm]{figures/transfer-learning-large-ltr.png}}                       & \begin{tabular}[c]{@{}l@{}}\textcolor[rgb]{0.141,0.161,0.18}{Trains weights on }\\\textcolor[rgb]{0.141,0.161,0.18}{layers and softmax }\\\textcolor[rgb]{0.141,0.161,0.18}{by initializing }\\\textcolor[rgb]{0.141,0.161,0.18}{weights on }\\\textcolor[rgb]{0.141,0.161,0.18}{pre-trained ones}\end{tabular}  \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Test}
\label{table:transfer_learning_strategy}
\end{table}

==> tables/unsupervised_training.tex <==
% \usepackage{multirow}

\begin{table}[!ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multicolumn{4}{|c|}{Pre-training}                                                                                                                                                   & Fine-tuning             & \multicolumn{2}{c|}{WER [\%]}  \\ 
\hline
\multirow{2}{*}{Architecture} & \multirow{2}{*}{Init}   & \multirow{2}{*}{Data (hours)}                                                                    & \multirow{2}{*}{Epochs} & \multirow{2}{*}{Epochs} & \multicolumn{2}{c|}{Viet.}     \\ 
\cline{6-7}
                              &                         &                                                                                                  &                         &                         & dev  & test                    \\ 
\hline
\multirow{7}{*}{\textit{Large}\textsubscript{1-8}\xspace}          & \multirow{5}{*}{random} & None                                                                                             & None                    & 33                      & 32.1 & 36.6                    \\ 
\cline{3-7}
                              &                         & \begin{tabular}[c]{@{}c@{}}Respective \\in-house data\\ Viet. (219h)\end{tabular}                & 100                     & \multirow{9}{*}{26}     & 31.4 & 33.4                    \\ 
\cline{3-4}\cline{6-7}
                              &                         & \begin{tabular}[c]{@{}c@{}}Viet. YT \\(1168h)\end{tabular}                                       & \multirow{3}{*}{300}    &                         & 29.8 & 35.2                    \\ 
\cline{3-3}\cline{6-7}
                              &                         & \begin{tabular}[c]{@{}c@{}}Viet. in-house + YT \\(1168h)\end{tabular}                            &                         &                         & 25.3 & 27.2                    \\ 
\cline{3-3}\cline{6-7}
                              &                         & \begin{tabular}[c]{@{}c@{}}Multilingual in-house \\(1168h)\end{tabular}                          &                         &                         & 26.8 & 28.7                    \\ 
\cline{2-4}\cline{6-7}
                              & \multirow{2}{*}{\textit{XLSR-53}\textsubscript{1-8}\xspace}    & None                                                                                             & None                    &                         & 27.6 & 31.9                    \\ 
\cline{3-4}\cline{6-7}
                              &                         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Respective in-house \\data Viet. (219h)\end{tabular}} & 25                      &                         & 27.6 & 29.5                    \\ 
\cline{1-2}\cline{4-4}\cline{6-7}
\textit{Large}\xspace                           & \textit{XLSR-53}\xspace                     &                                                                                                  & 100                     &                         & 26.2 & 29.0                    \\ 
\cline{1-4}\cline{6-7}
\multirow{2}{*}{\textit{Large}\textsubscript{1-8}\xspace}          & \multirow{2}{*}{\textit{XLSR-53}\textsubscript{1-8}\xspace}    & \begin{tabular}[c]{@{}c@{}}Viet. YT \\(1168h)\end{tabular}                                       & 100                     &                         & 24.3 & 28.1                    \\ 
\cline{3-4}\cline{6-7}
                              &                         & \begin{tabular}[c]{@{}c@{}}Multilingual in-house \\(1168h)\end{tabular}                          & 50                      &                         & 23.9 & 27.4                    \\
\hline
\end{tabular}
\caption{\glspl{WER} {[}\%{]} for models using unsupervised pre-training. All fine-tunings use the \textit{Large}\textsubscript{1-8} architecture and are trained until full convergence on the in-house data of the respective language. Pre-trainings have been done with random initialization or using the public \textit{XLSR-53}  checkpoint as initialization. Pre-training "None" means fine-tuning from scratch.}
\label{table:unsupervised_training}
\end{table}
